Toward Autonomous Rotation-Aware Unmanned Aerial Grasping

Autonomous Unmanned Aerial Manipulators (UAMs) have shown promising potentials to transform passive sensing missions into active 3-dimension interactive missions, but they still suffer from some difficulties impeding their wide applications, such as target detection and stabilization. This letter presents a vision-based autonomous UAM with a 3DoF robotic arm for rotational grasping, with a compensation on displacement for center of gravity. First, the hardware, software architecture and state estimation methods are detailed. All the mechanical designs are fully provided as open-source hardware for the reuse by the community. Then, we analyze the flow distribution generated by rotors and plan the robotic arm's motion based on this analysis. Next, a novel detection approach called Rotation-SqueezeDet is proposed to enable rotation-aware grasping, which can give the target position and rotation angle in near real-time on Jetson TX2. Finally, the effectiveness of the proposed scheme is validated in multiple experimental trials, highlighting it's applicability of autonomous aerial grasping in GPS-denied environments.

==> include/table.tex <==
\begin{tabular}{|l|c|c|c|c|}  
\hline  
\textbf{Link $i$} & \textbf{$a_i$} & \textbf{$\alpha_i$} & \textbf{$d_i$} & \textbf{$\theta_i$} \\\hline   
1                  & $L_1$          & 0                   & 0               &  \theta_1           \\\hline  
2                  & $L_2$          & 0                   & 0               & \theta_2             \\\hline  
\end{tabular}  


% company website
% www.hobbywing.com
% www.rcsunnysky.com
% www.nvidia.com
% www.intel.com
% www.smartsensor.cn
